Latent Clarity: Bridging World-Model Kinematics to Semantic Manifolds for Video Anomaly Anticipation

Continuous video anomaly detection is dominated by reactive Multiple Instance Learning (MIL) that collapses spatiotemporal features into scalar scores. We introduce PULS (Predictive Unified Latent Space), a continuous semantic world-model pipeline comprising two modules: a 490M-parameter KSD Bridge (Kinematic-to-Semantic Distillation) and a 16.8M-parameter Anticipatory State Predictor (ASP). The KSD Bridge maps V-JEPA 2 physical tensors into the 2048-d Qwen3-VL-Embedding-2B text-aligned hypersphere, trained on a subset of UCF-Crime. This translation alone yields a chunk-level AUROC of 0.8994 for UCF-Crime and 0.8162 for out-of-distribution XD-Violence without MIL or hierarchical fusion. We introduce and validate the Latent Clarity Hypothesis: because JEPA's temporal predictor discards aleatoric pixel noise while preserving kinematics, anticipated future representations are more semantically separable than observed presents. The ASP sharpens these anticipated future latents, achieving 44.5% mean 14-way zero-shot VQA accuracy (exceeding observation baseline by +9.6 pp). Applying the ASP to Observation Tensors collapses accuracy to 7.3% (random chance), proving Anticipation and Observation occupy distinct sub-manifolds. A Triple-Track Lead-Time protocol with an L1-surprise gate yields a peak +8.9 pp anticipatory advantage at T-0.5s (p < 0.001, N = 1,000 permutation), separating physical anticipation from static scene priors. Zero-shot transfer to XD-Violence confirms that Newtonian-invariant kinematic representations generalize out-of-distribution.

==> figures/fig3A_pipeline.tex <==
% fig3A_pipeline.tex — PULS Pipeline with ASP
% Usage: \input{figures/fig3A_pipeline} inside a figure environment

\usetikzlibrary{arrows.meta, positioning, fit, backgrounds, shapes.geometric}

\definecolor{nred}{RGB}{214,39,40}
\definecolor{ngreen}{RGB}{44,160,44}
\definecolor{nblue}{RGB}{31,119,180}
\definecolor{norange}{RGB}{255,127,14}
\definecolor{npurple}{RGB}{148,103,189}

\begin{tikzpicture}[
    >=Stealth,
    % Standardize box styles for crisp geometric presentation
    box/.style={rectangle, rounded corners=3pt, draw=gray!50, fill=gray!5, text centered, minimum width=2.4cm, minimum height=0.8cm, font=\small, align=center},
    frozen/.style={box, draw=nblue!60, fill=nblue!5, thick},
    trainable/.style={box, draw=norange!80, fill=norange!10, thick},
    tensor_obs/.style={box, draw=nred!60, fill=nred!5, thick},
    tensor_ant/.style={box, draw=ngreen!60, fill=ngreen!5, thick},
    arrow/.style={->, thick, draw=gray!80},
    ant_arrow/.style={->, thick, draw=ngreen!80},
    obs_arrow/.style={->, thick, draw=nred!80},
    loss_box/.style={box, draw=npurple!60, fill=npurple!5, thick}
]

% Row 0 (PULS L->R)
\node[tensor_ant] (z_ctx) at (0,0) {$\mathbf{Z}_{\mathrm{ctx}}$\\ \scriptsize (frames 1--8)};
\node[frozen] (vjepa) at (3.6,0) {\textbf{V-JEPA 2}\\ \scriptsize predictor};
\node[tensor_ant] (z_fut) at (7.2,0) {$\hat{\mathbf{Z}}_{\mathrm{future}}$};
\node[tensor_ant] (z_ant) at (10.8,0) {$\mathbf{Z}^{\mathrm{ant}}$\\ \scriptsize $[\mathbf{Z}_{\mathrm{ctx}} \parallel \hat{\mathbf{Z}}_{\mathrm{future}}]$};

% Row 1 (PULS R->L)
\node[tensor_ant] (s_sharp) at (0,-1.8) {$\mathbf{s}^{\mathrm{sharp}}$};
\node[trainable] (asp) at (3.6,-1.8) {\textbf{ASP}\\ \scriptsize trainable};
\node[tensor_ant] (s_blur) at (7.2,-1.8) {$\mathbf{s}^{\mathrm{blur}}$};
\node[frozen] (ksd_ant) at (10.8,-1.8) {\textbf{KSD Bridge}\\ \scriptsize frozen};

% Row 2 (ASP Training L->R)
\node[tensor_obs] (z_obs) at (3.6,-3.8) {$\mathbf{Z}^{\mathrm{obs}}$\\ \scriptsize $[\mathbf{Z}_{\mathrm{ctx}} \parallel \mathbf{Z}_{\mathrm{target}}]$};
\node[frozen] (ksd_obs) at (7.2,-3.8) {\textbf{KSD Bridge}\\ \scriptsize frozen (teacher)};
\node[tensor_obs] (s_obs) at (10.8,-3.8) {$\mathbf{s}^{\mathrm{obs}}$\\ \scriptsize (teacher)};

% Row 3 (Loss)
\node[loss_box, minimum width=4cm] (loss) at (7.2,-5.5) {\textbf{Loss}\\ $\mathrm{NCE}_{\mathrm{sym}}(\mathbf{s}^{\mathrm{sharp}},\mathbf{s}^{\mathrm{obs}})$};

% Backgrounds
\begin{scope}[on background layer]
    % PULS Box
    \node[fill=nblue!3, rounded corners, draw=nblue!20, dashed, fit=(z_ctx) (z_ant) (s_sharp) (ksd_ant), inner sep=0.4cm] (bg_puls) {};
    \node[anchor=south west, font=\bfseries\small, text=nblue] at (bg_puls.north west) {PULS Inference Track};
    
    % ASP Box
    \node[fill=nred!3, rounded corners, draw=nred!20, dashed, fit=(z_obs) (s_obs) (ksd_obs), inner sep=0.4cm] (bg_asp) {};
    \node[anchor=south west, font=\bfseries\small, text=nred] at (bg_asp.north west) {ASP Training Track};
\end{scope}

% Arrows PULS
\draw[ant_arrow] (z_ctx) -- (vjepa);
\draw[ant_arrow] (vjepa) -- (z_fut);
\draw[ant_arrow] (z_fut) -- (z_ant);

\draw[ant_arrow] (z_ant) -- (ksd_ant);

\draw[ant_arrow] (ksd_ant) -- (s_blur);
\draw[ant_arrow] (s_blur) -- (asp);
\draw[ant_arrow] (asp) -- (s_sharp);

% Arrows ASP
\draw[obs_arrow] (z_obs) -- (ksd_obs);
\draw[obs_arrow] (ksd_obs) -- (s_obs);

% Arrows Loss
\draw[->, thick, draw=npurple, rounded corners=6pt] (s_sharp.south) -- (0, -5.5) -- (loss.west);
\draw[->, thick, draw=npurple, rounded corners=6pt] (s_obs.south) -- (10.8, -5.5) -- (loss.east);

\end{tikzpicture}


==> figures/fig4_umap.tex <==
% fig4_umap.tex — UMAP cosine projection of ULSH embedding clouds
% [DEPRECATED] This figure has been absorbed into fig1_teaser.tex (panel c).
%              Kept as standalone reference; no longer \input'd from main.tex.
% Data from figures/data/umap_{obs,ant,cmp,anchor}.csv
% Generated by scripts/gen_umap_data.py
% Real data ranges: obs x[11.45,14.98] y[1.66,7.82] (right cluster, near anchors)
%                   ant x[-4.87,-0.28] y[0.28,4.68]  (left cluster)
%                   cmp x[-4.58,-0.57] y[0.67,4.65]  (co-located with ant)
%                   anchor x[11.04,11.13] y[4.19,4.32] (7 text anchors, right cluster)
%
% Usage: \input{figures/fig4_umap}  inside a figure environment

\definecolor{nblue}{RGB}{31,119,180}
\definecolor{nred}{RGB}{214,39,40}
\definecolor{ngreen}{RGB}{44,160,44}
\definecolor{norange}{RGB}{255,127,14}
\definecolor{ngray}{RGB}{127,127,127}

\begin{tikzpicture}
\begin{axis}[
  width=0.88\linewidth, height=7cm,
  xlabel={UMAP dim-1 (cosine metric)},
  ylabel={UMAP dim-2},
  xmin=-6, xmax=16,
  ymin=-1, ymax=9,
  grid=major, grid style={dashed, gray!15},
  legend style={font=\scriptsize, at={(0.02,0.98)}, anchor=north west,
                draw=black!30, fill=white, row sep=0pt},
  tick style={thin, black},
  title={\textbf{UMAP projection of ULSH embeddings}
         {\small (metric=cosine, $n{=}300$ obs, $n{=}300$ ant, $n{=}50$ CMP + 7 anchors)}},
]

% ---- Observation Tensors (right cluster, near text anchors) ----
\addplot[
  only marks, mark=o,
  mark options={fill=nred!30, draw=nred, opacity=0.6},
  mark size=1.5pt,
] table[x=x, y=y, col sep=comma]
  {figures/data/umap_obs.csv};
\addlegendentry{Observation ($\mathbf{Z}^{\mathrm{obs}}$)}

% ---- Anticipation Tensors (left cluster, distinct manifold) ----
\addplot[
  only marks, mark=triangle*,
  mark options={fill=ngreen!50, draw=ngreen!70!black, opacity=0.6},
  mark size=1.5pt,
] table[x=x, y=y, col sep=comma]
  {figures/data/umap_ant.csv};
\addlegendentry{Anticipation ($\mathbf{Z}^{\mathrm{ant}}$)}

% ---- Cross-Manifold Probe (co-located with ant region) ----
\addplot[
  only marks, mark=x,
  mark options={draw=norange, line width=1.2pt},
  mark size=2.5pt,
] table[x=x, y=y, col sep=comma]
  {figures/data/umap_cmp.csv};
\addlegendentry{Cross-Manifold Probe}

% ---- Text anchors (right cluster, 7 category prototypes) ----
\addplot[
  only marks, mark=star,
  mark options={fill=nblue, draw=nblue!70!black},
  mark size=4.0pt,
] table[x=x, y=y, col sep=comma]
  {figures/data/umap_anchor.csv};
\addlegendentry{Text anchors (7 XD categories)}

% ---- Cluster annotations ----
\node[font=\scriptsize, nred!80, anchor=south]
  at (axis cs:13.2,7.9) {obs / anchor};
\draw[nred!50, dashed, thick] (axis cs:11.2,1.4) rectangle (axis cs:15.2,8.0);

\node[font=\scriptsize, ngreen!70!black, anchor=north]
  at (axis cs:-2.5,-0.8) {ant manifold};
\draw[ngreen!50, dashed, thick] (axis cs:-5.1,0.0) rectangle (axis cs:0.1,5.0);

\end{axis}
\end{tikzpicture}


==> figures/puls_pipeline.tex <==
\begin{figure}[t]
\centering
\fbox{\parbox{0.95\linewidth}{\centering
\textbf{PULS inference:}\quad
$\mathbf{Z}_{\mathrm{ctx}}$ (frames 1--8)
$\xrightarrow{\text{V-JEPA\,2 temporal predictor}}\hat{\mathbf{Z}}_{\mathrm{future}}$
$\;\to\;\mathbf{Z}^{\mathrm{ant}} = [\mathbf{Z}_{\mathrm{ctx}} \,|\, \hat{\mathbf{Z}}_{\mathrm{future}}]$
$\xrightarrow{\text{frozen KSD Bridge}}\mathbf{s}^{\mathrm{blur}}$
$\xrightarrow{\text{ASP}}\mathbf{s}^{\mathrm{sharp}}$.\\[4pt]
\textbf{ASP training:}
$\mathbf{Z}^{\mathrm{obs}} = [\mathbf{Z}_{\mathrm{ctx}} \,|\, \mathbf{Z}_{\mathrm{target}}]$
$\xrightarrow{\text{frozen KSD Bridge}}\mathbf{s}^{\mathrm{obs}}$ (teacher).
Loss: $\mathrm{NCE}_{\mathrm{sym}}(\mathbf{s}^{\mathrm{sharp}},\mathbf{s}^{\mathrm{obs}})$.
}}
\caption{The PULS pipeline with ASP. Both teacher and student share the
same frozen KSD Bridge and the same present-tense query, isolating the
V-JEPA\,2 prediction error as the only learnable variable.}
\label{fig:puls}
\end{figure}

==> figures_ucf/fig_umap_ucf.tex <==
% fig_umap_ucf.tex — UMAP cosine projection of ULSH embeddings (UCF-Crime)
% Data from figures_ucf/data/umap_{obs,ant,cmp,anchor}_ucf.csv
% Generated by ucf_validation/ucf_gen_umap_data.py
%
% Real data ranges (2026-05-01 run):
%   obs  x[13.02,17.68]  y[2.42,8.50]   (right cluster)
%   ant  x[-4.27,0.95]   y[1.31,6.76]   (left cluster)
%   cmp  x[-3.95,0.62]   y[1.79,5.78]   (co-located with ant — proves context-only collapse)
%   anc  x[15.98,16.14]  y[11.49,11.65] (14 text anchors, upper-right)
%
% Usage: \input{figures_ucf/fig_umap_ucf}  inside a figure environment

\definecolor{nblue}{RGB}{31,119,180}
\definecolor{nred}{RGB}{214,39,40}
\definecolor{ngreen}{RGB}{44,160,44}
\definecolor{norange}{RGB}{255,127,14}
\definecolor{ngray}{RGB}{127,127,127}

\begin{tikzpicture}
\begin{axis}[
  width=0.88\linewidth, height=7cm,
  xlabel={UMAP dim-1 (cosine metric)},
  ylabel={UMAP dim-2},
  xmin=-5.5, xmax=19.5,
  ymin=-0.5, ymax=13.5,
  grid=major, grid style={dashed, gray!15},
  legend style={font=\scriptsize, at={(1.01,1.0)}, anchor=north west,
                draw=black!30, fill=white, row sep=0pt},
  tick style={thin, black},
  title={\textbf{UMAP projection of Semantic Latent States — UCF-Crime (in-distribution)}
         {\small (metric=cosine, 14 classes, obs vs.\ ant vs.\ CMP + 14 anchors)}},
]

% ---- Observation Tensors (Z^obs: context || actual_target) ----
\addplot[
  only marks, mark=o,
  mark options={fill=nred!30, draw=nred, opacity=0.6},
  mark size=1.5pt,
] table[x=x, y=y, col sep=comma]
  {figures_ucf/data/umap_obs_ucf.csv};
\addlegendentry{Observation ($\mathbf{Z}^{\mathrm{obs}}$)}

% ---- Anticipation Tensors (Z^ant: context || predicted_future) ----
\addplot[
  only marks, mark=triangle*,
  mark options={fill=ngreen!50, draw=ngreen!70!black, opacity=0.6},
  mark size=1.5pt,
] table[x=x, y=y, col sep=comma]
  {figures_ucf/data/umap_ant_ucf.csv};
\addlegendentry{Anticipation ($\mathbf{Z}^{\mathrm{ant}}$)}

% ---- Cross-Manifold Probe: context-only ablation [ctx | ctx] ----
\addplot[
  only marks, mark=x,
  mark options={draw=norange, line width=1.2pt},
  mark size=2.5pt,
] table[x=x, y=y, col sep=comma]
  {figures_ucf/data/umap_cmp_ucf.csv};
\addlegendentry{Cross-Manifold Probe}

% ---- Text Anchors (14 UCF-Crime category prototypes) ----
\addplot[
  only marks, mark=star,
  mark options={fill=nblue, draw=nblue!70!black},
  mark size=4.0pt,
] table[x=x, y=y, col sep=comma]
  {figures_ucf/data/umap_anchor_ucf.csv};
\addlegendentry{Text anchors (14 UCF classes)}

% ---- Cluster annotations ----

% obs cluster (right, mid-height)
\node[font=\scriptsize, nred!80, anchor=south]
  at (axis cs:15.35,8.7) {obs cluster};
\draw[nred!50, dashed, thick]
  (axis cs:12.0,1.8) rectangle (axis cs:18.3,9.0);

% ant + CMP manifold (left — CMP co-located proves context-only collapses)
\node[font=\scriptsize, ngreen!70!black, anchor=north]
  at (axis cs:-1.75,0.6) {ant\,/\,CMP manifold};
\draw[ngreen!50, dashed, thick]
  (axis cs:-5.0,0.8) rectangle (axis cs:1.6,7.3);

% text anchor cluster (upper right, isolated)
\node[font=\scriptsize, nblue!90, anchor=south west]
  at (axis cs:16.2,11.55) {text anchors};
\draw[nblue!40, dashed, thick]
  (axis cs:15.7,11.2) rectangle (axis cs:16.4,11.9);

\end{axis}
\end{tikzpicture}

